Superposed Random Spin Tensor Networks and their Holographic Properties

We study criteria for and properties of boundary-to-boundary holography in a class of spin network states defined by analogy to projected entangled pair states (PEPS). In particular, we consider superpositions of states corresponding to well-defined, discrete geometries on a graph. By applying random tensor averaging techniques, we map entropy calculations to a random Ising model on the same graph, with distribution of couplings determined by the relative sizes of the involved geometries. The superposition of tensor network states with variable bond dimension used here presents a picture of a genuine quantum sum over geometric backgrounds. We find that, whenever each individual geometry produces an isometric mapping of a fixed boundary region C to its complement, then their superposition does so iff the relative weight going into each geometry is inversely proportional to its size. Additionally, we calculate average and variance of the area of the given boundary region and find that the average is bounded from below and above by the mean and sum of the individual areas, respectively. Finally, we give an outlook on possible extensions to our program and highlight conceptual limitations to implementing these.

==> Chapters/01_Motivation.tex <==
\chapter{Motivation}

Introduction and the other shitty stuff.

==> Chapters/02_theory.tex <==
\chapter{Theoretical foundations}


\section{Polymer physics}






\section{Organic semiconductors}



\subsection{Electronic structure of $\pi$-orbital systems}




\subsection{Charge transport in organic semiconductors}



\paragraph{Band transport} $\;$ \\



\paragraph{Disordered transport models} $\;$ \\



\myFig[1\textwidth]{Graphics/Hopping}{Hopping}{This is the title of the figure}{this is the text describing the figure. "Hopping" in the brackets is the reference titel of the figure so that you can refer to it in the text}


\section{Field effect transistor}



\subsection{Metal-semiconductor and metal-insulator-semiconductor junctions}


\paragraph{Metal-semiconductor junction}


\paragraph{Metal-insulator-semiconductor junction}



\subsection{Current characteristics}

\paragraph{Linear regime}

\paragraph{Saturation regime}

\paragraph{Short channel effects}


\subsection{Organic FETs}

\paragraph{Thin film transistors}

\paragraph{Hysteresis}

\paragraph{Contact resistance effects}

\section{Ionic liquid gating}

==> Chapters/03_microscopy.tex <==
\chapter{Microscopy techniques}


\section{Polarized optical microscopy}

\myFig[0.7\textwidth]{Graphics/Microscopy2}{optmicro}{Polarized optical microscopy}{Incoming light is polarized and then reflected towards the sample by a beam splitter before it is focused and reflected by the substrate to be seen through the ocular}

There are several ways to uncover the alignment of the single polymers within the bulkfilm or the fiber. To identify the direction of alignment in this thesis optical microscopy was used. In particular a rotatable polarizer was installed in the optical path of the ingoing light. A detailed sketched is given in figure \ref{fig:optmicro}. The light is then reflected by a beam splitter towards the sample. Objectives with different magnifications were used to investigate the samples. The reflected light is then led to the ocular for observation with the eye or a digital camera. For pictures in this thesis a olympus system was used.


\section{Scanning electron microscopy}



\section{Atomic force microscopy}



==> Chapters/04_methods.tex <==
\chapter{Sample fabrication and methods}


\section{Microscopy techniques}

\subsection{Polarized optical microscopy}




\subsection{Atomic force microscopy}



\subsection{Scanning electron microscopy}


\section{Electronic layouts}





\section{Electron-beam lithography}




\subsection{Operation}



\subsection{Fabrication}



\section{Self assembled monolayers}



\subsection{SAMs for improved charge injection}


\subsection{Oxide covering SAMs}

==> Chapters/05_structure.tex <==
\chapter{Structural analysis of polymer films}


\section{Comparision}

==> Chapters/06_electricity.tex <==
\chapter{Electrical measurements}


\section{Charge transport measurements at ambient conditions}




\subsection{Setup}




\subsection{Measurements}





\section{Charge transport measurements in vacuum at different temperatures}

==> Chapters/07_discussion.tex <==
\chapter{Interpretation and discussion}

==> Chapters/08_summary.tex <==
\chapter{Summary and outlook}
